On the Weighted Quartet Consensus problem

In phylogenetics, the consensus problem consists in summarizing a set of phylogenetic trees that all classify the same set of species into a single tree. Several definitions of consensus exist in the literature; in this paper we focus on the Weighted Quartet Consensus problem, a problem with unknown complexity status so far. Here we prove that the Weighted Quartet Consensus problem is NP-hard and we give a 1/2-factor approximation for this problem. During the process, we propose a derandomization procedure of a previously known randomized 1/3-factor approximation. We also investigate the fixed-parameter tractability of this problem.

==> counterExample.eps_tex.tex <==
%% Creator: Inkscape inkscape 0.48.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'counterExample.eps' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{1240.34534083bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.28437796)%
    \put(0,0){\includegraphics[width=\unitlength]{counterExample.eps}}%
    \put(0.03468868,0.01500954){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$a$}}}%
    \put(0.26183257,0.11849595){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$a$}}}%
    \put(0.45652731,0.0807848){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$a$}}}%
    \put(0.68717921,0.01939456){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$a$}}}%
    \put(0.82136081,0.16848516){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$a$}}}%
    \put(0.12238902,0.27898757){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$b$}}}%
    \put(0.38022803,0.11761897){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$b$}}}%
    \put(0.48897642,0.06236775){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$b$}}}%
    \put(0.78715762,0.14042106){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$b$}}}%
    \put(0.99588446,0.10446392){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$b$}}}%
    \put(-0.00039146,0.1632231){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$c$}}}%
    \put(0.22149039,0.24390742){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$c$}}}%
    \put(0.57053778,0.18865621){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$c$}}}%
    \put(0.76523256,0.22461333){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$c$}}}%
    \put(0.90906113,0.25443145){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$c$}}}%
    \put(0.0162716,0.20531926){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$d$}}}%
    \put(0.32234581,0.20795028){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$d$}}}%
    \put(0.4232012,0.20093425){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$d$}}}%
    \put(0.61526492,0.22373634){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$d$}}}%
    \put(0.90643006,0.02290255){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$d$}}}%
    \put(0.07853884,0.00273147){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$e$}}}%
    \put(0.27498762,0.24566142){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$e$}}}%
    \put(0.54510467,0.10270987){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$e$}}}%
    \put(0.72839836,0.00010046){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$e$}}}%
    \put(0.8371468,0.21584332){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$e$}}}%
    \put(0.12940505,0.05885969){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$f$}}}%
    \put(0.21447438,0.19918025){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$f$}}}%
    \put(0.58720085,0.15006806){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$f$}}}%
    \put(0.77487963,0.06149071){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$f$}}}%
    \put(0.95729628,0.22549034){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$f$}}}%
    \put(0.86433383,0.04219663){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$g$}}}%
    \put(0.62666587,0.27021752){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$g$}}}%
    \put(0.41618505,0.16497711){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$g$}}}%
    \put(0.31445267,0.07903077){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$g$}}}%
    \put(0.16448508,0.16497711){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$g$}}}%
    \put(0.17325511,0.25443145){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$h$}}}%
    \put(0.36181085,0.07026073){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$h$}}}%
    \put(0.48108333,0.21145828){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$h$}}}%
    \put(0.97922129,0.05973669){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$h$}}}%
    \put(0.70121122,0.26846352){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$h$}}}%
  \end{picture}%
\endgroup%

